Modeling Design and Control Problems Involving Neural Network Surrogates

We consider nonlinear optimization problems that involve surrogate models represented by neural networks. We demonstrate first how to directly embed neural network evaluation into optimization models, highlight a difficulty with this approach that can prevent convergence, and then characterize stationarity of such models. We then present two alternative formulations of these problems in the specific case of feedforward neural networks with ReLU activation: as a mixed-integer optimization problem and as a mathematical program with complementarity constraints. For the latter formulation we prove that stationarity at a point for this problem corresponds to stationarity of the embedded formulation. Each of these formulations may be solved with state-of-the-art optimization methods, and we show how to obtain good initial feasible solutions for these methods. We compare our formulations on three practical applications arising in the design and control of combustion engines, in the generation of adversarial attacks on classifier networks, and in the determination of optimal flows in an oil well network.

==> AdversarialImages.tex <==
\section{Adversarial Attack Generation}

Deep neural networks have the immensely useful property of being able to uniformly approximate any function in a certain general class, but at the cost of being fairly opaque in terms of how the underlying machinery works.
This opacity may mask unpredictable behavior that makes these neural networks susceptible to attacks that disrupt the correct classifications observed on training and testing data.
\citep{szegedy2013intriguing} first demonstrated that almost imperceptible perturbations of image data may lead to misclassifications, in essence demonstrating key instabilities in neural networks. This work has led to a number of papers \citep{carlini2016evaluating, cheng2017maximum, fischetti2018deep} developing algorithms that produce estimates of the resilience of neural networks, estimating how close  an incorrectly classified image can be to a correctly classified one.

\subsection{Optimization Problem Formulation}

The central problem of interest as introduced by \citep{szegedy2013intriguing} is described as follows. Given a classifier $\text{DNN}$, an image $x \in [0,1]^m$, and a desired classification label $l$, we have the following problem.
\begin{equation}\label{eq:adversarialAttack}
\begin{array}{lll}
    \dps \mini_{z}\; & \|x - z\| & \\
    \st\; & \text{DNN}(z) =  l & \\
        & z \in [0,1]^m
\end{array}
\end{equation}
Essentially, we ask for an image of minimal distance to image $x$ that is classified with a different label. 

We add additional constraints (see, e.g., \citep{fischetti2018deep}) to ensure that this is a very confident classification. 
Specifically, we replace the constraint $\text{DNN}(z) = l$ with a constraint asking that the activation for label $l$ is some factor larger than the activation for each other label; in other words, if $y_L$ is the final layer, we have $y_{L,l} \ge \alpha y_{L,i}$ for $i \ne l$. 
Often  the final layer is given by applying a softmax function $y_{L,i} = \sigma(z_1,\ldots,z_n)_i = \exp(z_i)/\sum_j\exp(z_j)$ wherein the produced values effectively represent probabilities that the image is a given label.
In this case, we can represent this constraint in terms of $z_i$ as
\[
    \sigma(z)_l/\sigma(z)_i \ge \alpha \Leftrightarrow \exp(z_l - z_i) \ge \alpha \Leftrightarrow z_l \ge z_i + \log(\alpha),
\]
which is a linear constraint.
Then if we write $y_L = \text{DNN}(z)$ as the final layer prior to the softmax layer, we will have the following problem:
\begin{equation}\label{eq:adversarialAttack2}
\begin{array}{lll}
    \dps \mini_{z}\; & \|x - z\| & \\
    \st\; & y_L = \text{DNN}(z) & \\
        & y_L,l \ge y_L,i + \log(\alpha), \qquad i \ne l \\
        & z \in [0,1]^m .
\end{array}
\end{equation}
If we use the MINLP formulation from \eqref{eq:OptiDNN} for the $\text{DNN}$ constraints, then depending on our choice of
norm, it becomes an MILP (for $L^1$ or $L^{\infty}$ norms) or a mixed-integer quadratic program (for $L^2$ norm) that standard integer program solvers can handle. We will use the $L^2$ norm in experiments. If we use the NLP formulation from \eqref{eq:OptiDNN-NLP}, we will have a nonlinear program for use with any NLP solver.

We observe that the formulation in \eqref{eq:adversarialAttack2} is easily extendable and that constraints on the allowable perturbations can augment the formulation. For example, we may restrict the magnitude of the perturbation to any given pixel by restricting $|x_i - z_i| \le \epsilon$ for all $i$. Alternatively, we may be interested in continuous perturbations and therefore restrict $|(x_i - z_i) - (x_j - z_j)| < \epsilon$ for all pixels $j$ adjacent to pixel $i$.

\subsection{Experiments}

We assess the scalability and quality of solutions for all four formulations of \eqref{eq:adversarialAttack2} by considering adversarial attacks generated for the MNIST handwritten digit recognition data set \citep{lecun1998mnist}. We consider the 10 different architectures corresponding to having an input layer with $28\times28$ nodes followed by either 1 or 2 fully connected layers with 20, 40, 60, 80, or 100 hidden ReLU or Swish nodes each and then the output layer with 10 nodes and a softmax activation function. 

For each neural network, we train the model by minimizing the categorical cross entropy loss function for 10 epochs using the 60,000 digits of training data. Each neural network attains a test accuracy in 96--98\% when tested on the 10,000 digits of testing data.

We perform one solve of each formulation, and $\alpha$ set to $1.2$, meaning the probability for the given classification $l$ is 1.2 times higher than for any other. On each network, we solve the problem for 100 digits from the training data, with the goal of finding the closest image to the given digit that will be classified as a zero.  We run each iteration until convergence to the globally optimal solution (for the MIP formulation) or to a locally optimal solution (for the MPCC and embedded network formulations) or until one hour has passed, at which point we terminate with the best solution seen so far. We use CPLEX for the MIP formulation and Ipopt for the MCPP and embedded network formulations, and our computer setup is the same as before.

\subsection{Results}

In Table~\ref{tab:adversarial-results}, we tabulate the results of the experiments for the MIP and MPCC formulations. For each neural network architecture, we record the average solve times and objectives for CPLEX and Ipopt over the 100 solves. We also record how many times CPLEX finds the optimal solution and how many times it finds any solution, as well as how many times CPLEX finds a better solution than Ipopt.

%Architecture &  \pbox{2cm}{Mean \\ CPLEX \\ Time (s)} &  \pbox{2cm}{Mean \\ CPLEX \\ Obj.} &  \pbox{2cm}{\# Times \\CPLEX \\Finds \\Opt. Sol.} &  \pbox{2cm}{\# Times \\ CPLEX \\ Finds \\ Feas. Sol.} &  \pbox{2cm}{Mean \\IPOPT \\Time (s)} &  \pbox{2cm}{Mean \\IPOPT \\Obj.} &  \pbox{2cm}{\# Times \\CPLEX \\Wins} &  \pbox{2cm}{Mean \% \\Rel. Diff.\\ in Obj.} \\

\begin{table}
\centering
\begin{tabular}{lllllllll}
\toprule
Architecture &  \pbox{2cm}{Mean \\ MIP \\ Time (s)} &  \pbox{2cm}{Mean \\ MIP \\ Obj.} &  \pbox{2cm}{\# Times \\MIP \\Finds \\Opt. Sol.} &  \pbox{2cm}{\# Times \\ MIP \\ Finds \\ Feas. Sol.} &  \pbox{2cm}{Mean \\MPCC \\Time \\(s)} &  \pbox{2cm}{Mean \\MPCC \\Obj.} &  \pbox{2cm}{\# Times \\MIP \\Wins} &  \pbox{2cm}{Mean \% \\Rel. \\Diff.\\ in Obj.} \\
\midrule
784,20,10       & 1.82                & 1.79            & 100                               & 100                                & 0.34                & 1.80            & 100                 & 0.61                       \\
784,40,10       & 76.85               & 1.75            & 100                               & 100                                & 1.48                & 1.77            & 100                 & 0.95                       \\
784,60,10       & 2301.8             & 1.85            & 52                                & 100                                & 4.84                & 1.87            & 100                 & 1.04                       \\
784,80,10       & 2570.7             & 2.04            & 38                                & 100                                & 14.23               & 2.07            & 99                  & 1.24                       \\
784,100,10      & 3078.4             & 2.16            & 16                                & 100                                & 22.88               & 2.18            & 95                  & 0.94                       \\
784,20,20,10   & 106.1              & 1.20            & 100                               & 100                                & 0.82                & 1.22            & 100                 & 0.95                       \\
784,40,40,10   & 3100.0             & 1.90            & 16                                & 100                                & 4.39                & 1.77            & 98                  & 1.89                       \\
784,60,60,10   & 3513.1             & 6.85            & 5                                 & 100                                & 14.26               & 1.88            & 12                  & -41.13                     \\
784,80,80,10   & 3586.7             & 27.59           & 1                                 & 76                                 & 36.10               & 1.46            & 1                   & -77.85                     \\
784,100,100,10 & 3600             & 54.83           & 0                                 & 42                                 & 56.97               & 1.78            & 0                   & -92.98                    \\
\bottomrule
\end{tabular}
\caption{Comprehensive results for solves of the MIP formulation using CPLEX and the MPCC formulation using Ipopt}
\label{tab:adversarial-results}
\end{table}

Table \ref{tab:embedded-digit-results} describes the average objective and solve time for the best solutions found using the embedded ReLU and Swish Network formulations. It also lists the number of instances for which the solver fails to find a feasible solution (defined to be a solution which violates the constraints by at most $10^{-6}$) either due to failure to converge or convergence to an infeasible solution.

The average time to convergence for the CPLEX solves of the MIP formulation is significantly higher than that of the Ipopt solves of the MPCC formulation. Most CPLEX solves for the larger networks time out at 1 hour before finding an optimal solution; for the smaller networks, it can take 10 to 100 times longer to converge to a solution. Ipopt, on the other hand, takes less than a minute on average to converge to a locally optimal solution. The embedded formulations are fairly uniform in how long they take to find their best solution which makes sense given that the the problem does not change in size with the number of neurons in the network.

The longer solve times of the MIP formulation have the advantage of eventually uncovering better solutions the majority of the time even if they are not provably optimal. For all the single hidden layer architectures and the two smallest double hidden layer architecture, CPLEX almost always produces a better solution than Ipopt does. These solutions generally  offer only a marginal improvement on the order of 1--2\% difference in the objective. For perturbations of this magnitude, the differences are essentially imperceptible. Similarly, the embedded network formulations express marginal differences for better or worse in almost all cases.

\begin{table}
    \centering
\begin{tabular}{l|ccc|ccc}
\toprule
 & \multicolumn{3}{c}{Embedded ReLU Network} & \multicolumn{3}{c}{Embedded Swish Network} \\
Architecture &  Mean Obj. &  Mean Time &  \# Infeas. &  Mean Obj. &  Mean Time &  \# Infeas. \\
\midrule
784,20,10      &   1.94 &       23.6 &                 14 &    1.51 &        22.2 &                   8 \\
784,40,10      &   1.65 &       15.7 &                  1 &    1.81 &        17.5 &                   1 \\
784,60,10      &   2.06 &       13.6 &                  0 &    1.46 &        18.7 &                  10 \\
784,80,10      &   1.16 &       28.2 &                  7 &    1.72 &        10.1 &                   0 \\
784,100,10     &   1.78 &       21.2 &                  7 &    1.67 &         8.2 &                   0 \\
784,20,20,10   &   1.45 &       17.2 &                  3 &    1.50 &        29.4 &                   2 \\
784,40,40,10   &   1.75 &       19.6 &                  1 &    1.39 &        13.4 &                   0 \\
784,60,60,10   &   1.84 &       20.6 &                 13 &    1.29 &        15.1 &                   0 \\
784,80,80,10   &   1.48 &       20.2 &                  0 &    1.14 &        12.1 &                   0 \\
784,100,100,10 &   1.75 &       19.3 &                  0 &    2.07 &        12.9 &                   0 \\
\bottomrule
\end{tabular}
\caption{Results from 100 trials on the embedded network formulation using both ReLU functions and Swish activation functions.}
\label{tab:embedded-digit-results}
\end{table}

For the largest networks, the MIP formulation fares poorly and cannot find a feasible solution in all cases for the two largest networks. The feasible solutions it does find are of noticeably lower quality: CPLEX  has the better solution in only 13 cases out of 300 from the three largest networks. The MIP solutions for the larger networks are visually worse, as can be seen in a comparison between the perturbed images generated from CPLEX and Ipopt in Figure~\ref{fig:perturbed_digit_suite} with respect to the original images in Figure~\ref{fig:digit_suite}. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{images/digit_suite}
    \caption{Suite of 10 digits from the MNIST training data for which adversarial attacks are generated.}
    \label{fig:digit_suite}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{images/cplex_digit_suite}
    \includegraphics[width=0.45\linewidth]{images/ipopt_digit_suite}
    \caption{Perturbed images produced after 1 hour of computation when using CPLEX to solve the MIP formulation (left) and Ipopt to solve the NLP formulation (right) with given digits in Figure~\ref{fig:digit_suite} for the neural network with 2 hidden layers of 100 nodes}
    \label{fig:perturbed_digit_suite}
\end{figure}

When compared to the MIP and MPCC formulations, the embedded formulations while often faster and more scalable, can be more unstable in the sense that they can fail to find feasible solutions even though for this problem, they certainly exist. The ReLU networks are more prone to failure and exhibit the ill-posed behavior as in Figure \ref{fig:dual-infeas} leading to failure to find solutions in about 5\% of instances. The Swish networks are better behaved but still fail to find a single feasible solution in about 2\% of cases.

==> EngineDesign.tex <==
\section{Optimal Design of Combustion Engines}\label{sec:engine}

Automobile engine operation is typically modeled by using highly intensive physics-based simulation code, which even on powerful computers can take hours  for a short drive. Hence, modeling the evaluation of this simulation code by using a neural network surrogate model can produce significant time savings at the cost of producing slightly less accurate results. A study examining this approach is documented in \citep{aithal2019maltese}.

Given this neural network, we could formulate several optimization problems answering questions related to the operation of an engine on a given commute. A natural problem one might have is that  of minimizing emissions over the course of a given drive. The resulting solution would then be both the engine type and the drive style (e.g., RPM at all times in the drive) that produces the most environmentally efficient commute. The following section demonstrates how such a problem can be formulated.

\subsection{A Simple Engine Design and Control Problem}
Suppose we have a trained DNN that predicts engine behavior based on engine specifications and driving parameters, given in Table \ref{tab:engineDNN}. The DNN is trained by using 64 trips each split into 1,500 observations (25 minutes observed at second intervals).

\begin{table}[htbp]
    \centering
    \begin{tabular}{l||l}
    Input Parameter and Output Parameter \\ \hline
    fuel injection (g) /s      &  NO /s \\
    engine RPM     /s      &  CO /s  \\
    compression ratio     &  torque /s \\
%    ambient temperature /s &  exhaust pressure /s \\
%    ambient pressure    /s &  peak engine temperature \\
%                           &  peak engine temperature\\ \hline
    \end{tabular}
\caption{Input/output parameters of engine DNN model. Time-dependent parameters are shown with time per second (/s).}
\label{tab:engineDNN}
\end{table}

The problem we propose to solve is the optimal design and control of an engine for a given 25-minute trip. We will use a prescribed torque profile as a surrogate for the trip characteristics and minimize a weighted sum of NO and CO output. Our optimization variables are fuel injection, $f$; engine RPM, $r$; and compression ratio, $c$. Formally, we state  the following optimal design and control problem over the time horizon $t=1,\ldots,T$ (where $T=1500$ is the number of seconds):
\begin{equation}\label{eq:optEngine}
    \begin{array}{lll}
        \dps \mini_{f,r,c} & \dps \sum_{t=1}^T (\text{NO}(t) + \lambda \text{CO}(t))\Delta t \qquad & \text{min. NO and CO emissions} \\
        \st & \text{Torque}(t) \geq \text{PrescribedTorque}(t), \; \forall t=1,\ldots,T \qquad & \text{trip profile} \\
          & \left( \text{NO}(t), \text{CO}(t), \text{Torque}(t) \right) = \text{DNN}\left( f(t), r(t), c \right) & \text{DNN constraints} \\
          & f(t) \in [f_{\min}, f_{\max}], \; r(t) \in [r_{\min}, r_{\max}], \; c \in [c_{\min}, c_{\max}] & \text{bounds on controls}.
    \end{array}
\end{equation}
We abbreviate the collection of DNN constraints and note that this problem may represent either the MINLP formulation \eqref{eq:OptiDNN} or the NLP formulation \eqref{eq:OptiDNN-NLP}. We remark that the last layer has no ReLU nodes since the output of the neural network may take all real values. Note that since the objective and all constraints (apart from DNN constraints) are linear, the MINLP formulation is in fact a mixed-integer linear program (MILP), and we will refer to it as such.

We will discretize this problem using the same 1,500 time points as in the DNN model.  Note that as the problem is written, we will have $3T$ continuous control variables in addition to the variables that encode the deep neural network. 
Our model has a separate DNN evaluation for each time step $t$, resulting in an optimization problems with $T$ different sets of variables for each DNN evaluation. Because of the presence of the design parameter $c$, which is independent of $t$, this problem  does not decompose into
individual time steps.
In the MILP formulation, since each hidden node has an ReLU activation function, the number of binary variables is given by $(\# \text{Hidden Nodes})\times T$, which quickly grows beyond the scope of most general solvers as $T$ increases.

% \subsection{A Simple Engine Inverse Problem}

% Given that the engine design problem quickly becomes computationally intractable as the number of layers and the number of time steps increase, we can consider alternate problems which are hopefully easier to solve. Consider instead the inverse problem described in the introduction. We could very well be given a time series of emissions data from an engine and ask what type of engine could possibly produce these emissions, at least according to our neural network. 

% If we have a sample of these output values at specific times, we may adapt our original optimization problem to the following:

% \begin{equation}\label{eq:invEngine}
%     \begin{array}{lll}
%         \dps \mini_{f,r,c} & \dps \sum_t\|\text{NOx}(t) - \widehat{\text{NOx}}(t)\|^2 + \|\text{CO}(t) - \widehat{\text{CO}(t)} \|^2 \qquad & \text{min. NOx and CO emissions} \\
%           & \left( \widehat{\text{NOx}}, \widehat{\text{CO}} \right) = \text{DNN}\left( f, r, c \right) & \text{DNN constraint} \\
%           & f(t) \in [8, 32], \; r(t) \in [800, 3000], \; c \in [9.5, 10.5] & \text{bounds on controls}.
%     \end{array}
% \end{equation}

% We distinguish the observed NOx and CO from the estimated NOx and CO using the neural network by giving hats to the latter. Note that this model can easily be extended to include more input and output parameters should we have a more involved neural network model.

\subsection{Convex-Hull Constraints}

In addition to the constraints that encode the evaluation of a neural network,  constraints must be added to ensure that the solver does not extrapolate significantly from the training data. 
Without these constraints, the optimization routine may find that the optimal solutions resides in an area for which the neural network has not learned the behavior of the modeled function leading to a solution that, while optimal, does not reflect true function behavior and may be nonsensical. 
In fact, in an earlier implementation without the convex-hull constraint, we observed that the optimal design 
was obtained for an engine that produced negative emissions. 
We rectify this error by introducing constraints that constrain the input data to our model to be within the convex hull of the input training data. 

In our experiments, we examined how the optimization models operated with simple box constraints that bounded the input by the extremal values of the training data, as well as with the convex hull constraints. Figure~\ref{fig:convex-hull} demonstrates the location of fuel mass and RPM for solutions computed for a sample neural network trained on our data set compared with the actual training data. The corresponding solutions are displayed in Figure~\ref{fig:convex-hull-solutions}.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.45\linewidth]{images/no_hull_constraints_1.png}
    \includegraphics[width=0.45\linewidth]{images/hull_constraints_1.png}
     \caption{Location of training data and optimal solution for an engine design problem on a neural network with 1 hidden layer of 16 nodes. On the left, the input is constrained by box constraints and on the right by convex-hull constraints.}
    \label{fig:convex-hull}
\end{figure}

Without the convex hull constraints, the optimal solution of neural network evaluation appears to wander off to an area for which there is no training data. 
This immediately creates problems in the computed solutions, which are obviously nonsensical because of involving negative emissions. This suggests that our neural network does not generalize well to data that has not yet been seen by the network. 
On the other hand, constraining the input data to be within the convex hull has the effect of producing solutions that look like the training data.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.45\linewidth]{images/layer_1_solution.png}
    \includegraphics[width=0.45\linewidth]{images/layer_1_solution_hull.png}
    \caption{Optimal configuration for each time step when using box constraints (left) and using convex-hull constraints (right). The red lines indicate the drive cycles used to train the neural network, and the blue lines indicate the optimal solution.}
    \label{fig:convex-hull-solutions}
\end{figure}

Unfortunately, these constraints have the effect of restricting possible solutions to those that are close to the training data, when the function being modeled may have a minimum that appears far from the training data. 
This situation speaks to the limitations of using solely a surrogate model for optimization. To find a global optimum of the original function would necessarily involve an alternating approach wherein the surrogate model was optimized and then this solution was queried against the modeled function for new data to be added to the surrogate. 
This type of approach is addressed in \citep{queipo2005surrogate}.

If we fix the compression ratio, we can plot the contours of the objective function
as a function of fuel mass and RPM. Figure~\ref{fig:contour} shows the contours of the objective function for a
5-layer DNN. We observe that this objective function is highly nonconvex in the reduced space of the original 
variables but it is convex in the lifted MINLP space according to Proposition~\ref{prop:ConvexDNN}. We also 
observe that the convex-hull constraint fulfills a second function by acting as a mild convexifier of the 
problem by restricting the variables to a small sliver of the feasible set.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{images/contour_5_16.png}
    \caption{Contour plot for the NO output of a 5-layer DNN.}
    \label{fig:contour}
\end{figure}

\subsection{Warmstarting the Problem}

Seeding a MILP or NLP solver with a feasible solution of high quality can  significantly reduce the solve time. 
For MILP solvers, a feasible solution with sufficiently low value can be used to prune subproblems with  higher objective value in a branch-and-bound tree search. 
For NLP solvers, beginning with a feasible solution avoids the need to search for a feasible solution, and the choice of a good solution can ensure quicker convergence to better locally optimal solutions.

For the optimal engine design problem, we can use our collection of training data to find parameterizations of the engine that exceed the desired torque value but also have a low amount of emissions produced. We do not directly work with the output data from the training set but rather with the output from the neural network applied to the input data since this is what is constrained.

To produce a high-quality solution is then a matter of fixing the parameters that must remain constant for the entire drive (i.e., the compression ratio) and then, from the training data with these fixed parameters, choosing the remaining controls so as to minimize emissions while still exceeding the desired torque for each time step. The remaining variable values correspond to activation of each neuron in the neural network when applied to the input data and hence must be set to exactly those values. This procedure is summarized in Algorithm~\ref{alg:warmstart}.

\begin{algorithm}
    \caption{Algorithm for finding a warmstart solution to \eqref{eq:optEngine}}
    \label{alg:warmstart}
    \KwData{Input $\text{DNN}$, compression ratio $c_0$, training data $\mathcal{X}$, torque profile $\text{TorqueProfile}_t$, $T$}
    Select subset of training data $\tilde{\mathcal{X}}$ with compression ratio $c_0$\;
    Let $\tilde{\mathcal{Y}} = \text{DNN}(\tilde{\mathcal{X}})$\;
    \For{$t=1,\ldots,T$}{
        Let $\text{NO}, \text{CO}, \text{Torque} = \tilde{\mathcal{Y}}$\;
        Let $\mathcal{T}$ be the set of times $t$ where $\text{Torque}_t \ge \text{TorqueProfile}_t$\;
        Let $\tau = \text{argmin}_{t\in\mathcal{T}} (NO_t + \lambda CO_t)$\;
        Let $x_t = \tilde{\mathcal{X}}_\tau$\;
    }
    Set remaining variable values from activation of DNN when applied to $x_t$ for all $t$.\;
\end{algorithm}

% \subsection{Decomposing over Time}

% The problems described in (\ref{eq:optEngine}) and (\ref{eq:invEngine}) suffer on larger time scales as each time step of the model corresponds to a separate evaluation of the neural network and therefore another set of binary variables. The number of binary variables in a network corresponds exactly to the number of ReLU activation function applications. For our design and inverse problems, then the total number of binary variables is given by $\#\text{ binary variables} = (\#\text{ timesteps})(\#\text{ ReLU nodes})$.

% Our problem would become significantly easier should we be able to decompose the problem over time. We note that if we fix the compression ratio to $c^*$, then we can solve the following problem for each time step $t^*$ and sum up the computed solutions.
% \begin{equation}\label{eq:EngineSubproblem}
%     \begin{array}{ll}
%     \mini_{f,r} \quad & \text{NOx} + \lambda \text{CO} \\
%     \st \quad & \text{Torque} \ge \text{PrescribedTorque}(t^*) \\
%         & (\text{NOx}, \text{CO}, \text{Torque}) = \text{DNN}(f,r,c^*) \\
%         & f \in [8, 32], r \in [800, 3000]
%     \end{array}
% \end{equation}
% We note that most solvers provide dual values for when we add a constraint fixing $c = c^*$ which tell us in which direction we need to adjust the value of $c$ so as to decrease the objective value. Since we will be solving $T$ of these subproblems, we simply sum the dual values from each to get the direction for which we will proceed.

% We have the following bilevel optimization problem:

% \begin{align}\label{eq:decEngine}
%     \mini_{c} \quad &\sum_{t=0}^T (\text{NOx}(t) + \lambda\text{CO}(t))dt \\
%     \st \quad & \text{NOx}(t) + \lambda\text{CO}(t) \text{ a solution to } \eqref{eq:EngineSubproblem} \text{ at } (c,t), \forall t \in \{0,\ldots,T\} \\
%         & c \in [9.5,10.5]
% \end{align}

% This type of formulation leads to a very natural algorithm for finding the locally optimal solutions presented in Figure \ref{alg:decomposedAlg}.

% \begin{figure}
% \begin{algorithmic}
%     \STATE Input $DNN, T, c_0, \epsilon$
%     \STATE Initialize $c \gets c_0$
%     \WHILE{True}
%         \STATE Solve subproblem for given $DNN$ for $(t, c)$ for all $t =1,\ldots,T$
%         \STATE Recover $(f_t), (r_t), (NOx_t), (CO)_t$ from solver for each $t$ 
%         \STATE Recover dual variables $\lambda_t$ for each $t$.
%         \STATE Set $\Delta c \gets \sum_t \lambda_t$
%         \STATE Set $c \gets c + \mu \Delta c$
%         \IF{$|\Delta c| < \epsilon$}
%             \RETURN Solution $(f_t), (r_t), c, (NOx_t), (CO_t)$
%         \ENDIF
%     \ENDWHILE
% \end{algorithmic}
% \caption{Algorithm for finding local optima of (\ref{eq:decEngine})}
% \label{alg:decomposedAlg}
% \end{figure}

\subsection{Experiments}

We have applied these algorithms to a collection of neural networks with varying numbers of layers to study how well each formulation scales. 
The architectures we tested all have the simple structure of an input layer with the three input variables, followed by $n$ hidden layers of 16 nodes, and then the output layer with the three output variables. 
We consider networks with 1, 3, and 5 hidden layers and train each of these networks  for 20 epochs on the simulation data produced by the simulator of \citep{aithal2019maltese}.

Solving the MIP to optimality is generally intractable (even for a single-layer network, this amounts to $1500*16*1 = 24000$ binary variables, beyond the scope of any general-purpose state-of-the-art solver), so we consider instead a coarser discretization using larger time steps.

Instead of reading in the data at each second as is presented in the original data, we consider time steps of 750, 500, 250, 150, 30, 15, 10, 5, and 1 seconds. 
Since we have 1,500 seconds of data, this corresponds to 3, 6, 10, 50, 100, 150, 300, and $1500$ time steps for which we are evaluating our neural network. 
At each of the larger time steps, our prescribed torque profile will be the average of the prescribed torques in that interval. This approach gives us separate problems for each choice of coarseness of the discretization and for each choice of neural network architecture.

We assess the performance of solvers for both the MIP and MPCC formulations of \eqref{eq:optEngine}. 
We use the commercial solver CPLEX \citep{cplex12} to solve the MIP formulation of the problem and the solver Ipopt \citep{wachter.biegler:06} to solve the MPCC formulation of the problem. Both solvers are run with the default options. 
We run each of the solvers until they either converge to a solution or 3 hours pass, at which point the solve is terminated prematurely and the best-found solution so far is selected.

We also consider the embedded ReLU and Swish network formulations again using the solver Ipopt within the algebraic modeling language JuMP. 
For each instance, we run until convergence to a solution, 3 hours have passed or Ipopt has performed 3000 iterations. 
If the solver has not converged at the end of the experiment, we record the best solution discovered which has a constraint violation under $10^{-6}$.

All experiments are performed on a single thread on a Intel Xeon Gold 6130 CPU with 64 cores and 188 GB of memory.

\subsection{Results}

The amount of time needed solver until a solver found its best solution with a timem limit of 3 hours on each architecture with each timestep size is displayed in Table~\ref{tab:engine_times} with the corresponding objectives shown in Table~\ref{tab:engine_objs}.
%GAIL - note that here and for the next tble the capio os below, whereas for Tble 1 it was above. The usual placement ia above. I have left as is for you to decide.
% \begin{table}
%     \centering
% \begin{tabular}{ll|rrrrrrrr}
% \toprule
%       &                                & \multicolumn{8}{c}{No. of Time Steps} \\
% Solver & \pbox{2cm}{No. of \\ Hidden \\Layers} &     3    &     6    &     10   &     50   &     100  &     150  &     300  &     1500 \\
% \midrule
% CPLEX & 1 &      0.2 &      1.0 &      8.9 &  10800 &  10800 &  10800 &  10800 &  10800 \\
%                 & 3 &   2359 &  10800 &  10800 &  10800 &  10800 &  10800 &  10800 &  10800 \\
%                 & 5 &  10800 &  10800 &  10800 &  10800 &  10800 &  10800 &  10800 &  10800 \\ \hline
% CPLEX  & 1 &      0.9 &      2.8 &     13.8 &  10800 &  10800 &  10800 &  10800 &  10800 \\
% Warmstart                & 3 &   1134.0 &  10800 &  10800 &  10800 &  10800 &  10800 &  10800 &  10800 \\
%                 & 5 &  10800 &  10800 &  10800 &  10800 &  10800 &  10800 &  10800 &  10800 \\ \hline
% Ipopt & 1 &      0.2 &      0.2 &      0.6 &      3.3 &     12.9 &     27.7 &     79.4 &   1286.4 \\
%                 & 3 &      0.4 &      1.1 &      2.4 &     45.6 &    111.5 &    304.2 &   1048.1 &   9285.6 \\
%                 & 5 &      0.5 &      2.2 &      4.9 &     94.4 &    211.9 &    343.7 &   1666.5 &   7871.0 \\ \hline
% Ipopt  & 1 &      0.2 &      0.3 &      0.3 &      3.3 &      6.9 &     14.3 &     48.6 &    347.9 \\ 
% Warmstart                & 3 &      0.3 &      0.6 &      2.6 &     21.8 &     78.2 &    157.0 &    587.2 &   8591.9 \\
%                 & 5 &      0.3 &      1.0 &      2.3 &     45.7 &    107.7 &    249.0 &    805.3 &  10039.6 \\
% \bottomrule
% \end{tabular}
%     \caption{Solve times for each solver on each architecture for varying values of $T$. A time of 10800 indicates that the solve reached its time limit.}
%     \label{tab:engine_times}
% \end{table}

\begin{table}[htbp]
    \centering

\begin{tabular}{lc|rrrrrrrr}
\toprule
       &                                & \multicolumn{8}{c}{No. of Time Steps} \\
Formulation & \pbox{2cm}{No. of \\ Hidden \\Layers} &     3    &     6    &     10   &     50   &     100  &     150  &     300  &     1500 \\
\midrule
MIP & 1 &      0.2 &      1.0 &      8.9 &  $9530^*$ &  $9759^*$ &  $10252^*$ &  $10800^*$ &  $10800^{*\dagger}$ \\
                & 3 &   2359 &  $9749^*$ &  $10800^{*\dagger}$ &  $10800^{*\dagger}$ &  $10800^{*\dagger}$ &  $10800^{*\dagger}$ &  $10800^{*\dagger}$ &  $10800^{*\dagger}$ \\
                & 5 &  $1969^*$ &  $9501^*$ &  $10800^{*\dagger}$ &  $10800^{*\dagger}$ &  $10800^{*\dagger}$ &  $10800^{*\dagger}$ &  $10800^{*\dagger}$ &  $10800^{*\dagger}$ \\ \hline
MIP  & 1 &      0.9 &      2.8 &     13.3 &  $9673^*$ &  $9839^*$ &  $4363^*$ &  $10741^*$ &  $10304^*$ \\
Warm-                & 3 &  1100  &  336 &  $9763^*$ &  $10309^*$ &  $10800^*$ &  $10610^*$ &  $10485^*$ &  $10800^{*\dagger}$ \\
start                & 5 &  $1969^*$ &  $10800^{*\dagger}$ &  $1829^*$ &  $10332^*$ &  $10800^{*\dagger}$ &  $10800^{*\dagger}$ &  $10800^{*\dagger}$ &  $10800^{*\dagger}$ \\ \hline
MPCC & 1 &      0.2 &      0.2 &      0.6 &      3.3 &     12.9 &     27.7 &     79.4 &   1286.4 \\
                & 3 &      0.4 &      1.1 &      2.4 &     45.6 &    111.5 &    304.2 &   1048.1 &   9285.6 \\
                & 5 &      0.5 &      2.2 &      4.9 &     94.4 &    211.9 &    343.7 &   1666.5 &   7871.0 \\ \hline
MPCC  & 1 &      0.2 &      0.3 &      0.3 &      3.3 &      6.9 &     14.3 &     48.6 &    347.9 \\ 
Warm-                & 3 &      0.3 &      0.6 &      2.6 &     21.8 &     78.2 &    157.0 &    587.2 &   8591.9 \\
start                & 5 &      0.3 &      1.0 &      2.3 &     45.7 &    107.7 &    249.0 &    805.3 &  10040 \\
\bottomrule
\end{tabular}
\caption{Time until a solver found its best solution within 3 hours on each architecture for varying values of $T$. A $*$ indicates that a CPLEX solve did not finish within 3 hours meaning the found solution is not necessarily optimal. A $\dagger$ indicates CPLEX did not find any feasible solutions within 3 hours (except for the warmstart solution when it was used).}
\label{tab:engine_times}
\end{table}


\begin{table}[htbp]
    \centering
\begin{tabular}{lc|rrrrrrrr}
\toprule
       &                                & \multicolumn{8}{c}{No. of Time Steps} \\
Formulation & \pbox{2cm}{No. of \\ Hidden\\ Layers} &     3     &   6       &   10       &  50       &  100       & 150        &    300     & 1500        \\
\midrule
MIP & 1 &  6787 &  6785 &  6836 &  6923 &  6929 &  6932 &  7338 &     NaN \\
                & 3 &  7020 &  7013 &  7042 &     NaN &     NaN &     NaN &     NaN &     NaN \\
                & 5 &  6855 &      NaN &      NaN &     NaN &     NaN &     NaN &     NaN &     NaN \\ \hline
MIP  & 1 &  6787 &  6785 &  6836 &  6923 &  6929 &  6932 &  6984 &  7046 \\
Warmstart                & 3 &  7020 &  7013 &  7042 &  7077 &  7079 &  7083 &  7083 &  7084  \\
                & 5 &  6855 &  6911 &  6920 &  7047 &  7072 &  7072 &  7058 &  7073 \\ \hline
MPCC & 1 &  6787 &  7199 &  6839 &  6923 &  6930 &  6932 &  6932 &  6932  \\
                & 3 &  7088 &  7087 &  7119 &  7114 &  7126 &  7117 &  7114 &  7091 \\
                & 5 &  7082 &  7100 &  7194 &  7322 &  7242 &  7243 &  7333 &  7245  \\ \hline
MPCC & 1 &  6787 &  6785 &  6839 &  6923 &  6930 &  6933 &  6931 &  6932 \\
Warmstart       & 3 &   7041 &  7013 &  7041 &  7077 &  7081 &  7082 &  7081 &  7082 \\
                & 5 &  6855 &  6894 &  6920 &  7037 &  7045 &  7047 &  7048 &  7048  \\
\bottomrule
\end{tabular}
\caption{Computed objective values (total emissions output in 1000s of ppm) for each solver on each architecture for varying values of $T$. A ``NaN'' value  indicates that no feasible solution was found within 3 hours.}
\label{tab:engine_objs}
\end{table}

\begin{table}
\centering
\begin{tabular}{lc|rrrrrrrr}
\toprule
       &                                & \multicolumn{8}{c}{No. of Time Steps} \\
Formulation & \pbox{2cm}{No. of \\ Hidden\\ Layers} &     3     &   6       &   10       &  50       &  100       & 150        &    300     & 1500        \\
\midrule
Embedded  & 1 &   0.7 &   2.5 &  16.0 &   11.9 &    4.1 &   15.1 &     6.0 &    29.8 \\
ReLU Network                        & 3 &  21.8 &  21.9 &  74.2 &   88.9 &  195.2 &  408.4 &   157.2 &  3520.4 \\ 
                         & 5 &  21.9 &  23.0 &  67.6 &  223.3 &  395.7 &  315.0 &  1275.7 &  2469.2 \\ \hline
Embedded & 1 &   3.1 &   2.1 &  29.9 &    5.1 &   17.1 &   54.2 &    18.1 &    68.1 \\
ReLU Network                         & 3 &  17.7 &  12.4 &   5.3 &  196.2 &    5.7 &   44.5 &   252.8 &   485.5 \\
Warmstart                         & 5 &  26.1 &   $0.0^*$ &  $0.0^*$ &  130.2 &    $0.0^*$ &    $0.0^*$ &     $0.0^*$ &     $0.0^*$ \\ \hline
Embedded  & 1 &   4.2 &   3.7 &   4.6 &    7.4 &   17.1 &   27.7 &   271.3 &   793.5 \\
Swish Network                        & 3 &   6.9 &   7.4 &   8.0 &   10.0 &   35.5 &   21.6 &    50.2 &   550.7 \\
                         & 5 &   7.1 &   7.5 &   7.5 &    8.9 &   11.2 &   13.3 &    16.7 &    32.5 \\ \hline
Embedded & 1 &   4.4 &   3.1 &   3.2 &    5.9 &    6.5 &   10.7 &    23.3 &   193.2 \\
Swish Network                         & 3 &   6.5 &   5.6 &   7.2 &    9.7 &   14.9 &   20.4 &    34.1 &   149.9 \\
Warmstart                         & 5 &   7.8 &   7.1 &   7.2 &    8.8 &    9.9 &   10.6 &    17.2 &    32.7 \\

\bottomrule
\end{tabular}
\caption{The amount of time until Ipopt found its best solution for the embedded formulations within a time limit of 3 hours. An * indicates that Ipopt did not find any solution better than the warmstart solution.}
\label{tab:embedded-engine-time}
\end{table}

\begin{table}
\centering
\begin{tabular}{lc|rrrrrrrr}
\toprule
       &                                & \multicolumn{8}{c}{No. of Time Steps} \\
Formulation & \pbox{2cm}{No. of \\ Hidden\\ Layers} &     3     &   6       &   10       &  50       &  100       & 150        &    300     & 1500        \\
\midrule
Embedded  & 1 &  6787 &  6785 &  6836 &  6923 &  7317 &  7320 &  7320 &  7320 \\
ReLU Network                         & 3 &  7020 &  7013 &  7039 &  7079 &  7296 &  7297 &  7129 &  7403 \\
                         & 5 &  6878 &  6919 &  6963 &  7233 &  7557 &  7505 &  7533 &  7781 \\ \hline
Embedded & 1 &  6787 &  6785 &  6836 &  6923 &  6930 &  6932 &  6932 &  6932 \\
ReLU Network                         & 3 &  7020 &  7012 &  7039 &  7076 &  7079 &  7080 &  7081 &  7082 \\
Warmstart                         & 5 &  6878 &  6911 &  6956 &  7037 &  7072 &  7072 &  7072 &  7073 \\ \hline
Embedded  & 1 &  7065 &  7034 &  6956 &  7036 &  7101 &  7085 &  7171 &  7073 \\
Swish Network                         & 3 &  7466 &  7468 &  7439 &  7085 &  7468 &  7495 &  7391 &  7404 \\
                         & 5 &  6798 &  6786 &  6798 &  6860 &  6865 &  6868 &  6867 &  6867 \\ \hline
Embedded & 1 &  6908 &  6911 &  6971 &  7040 &  7037 &  7041 &  7039 &  7039 \\
Swish Network                         & 3 &  6895 &  6907 &  6964 &  7056 &  7062 &  7065 &  7067 &  7068 \\
Warmstart                         & 5 &  6798 &  6786 &  6798 &  6889 &  6887 &  6896 &  6891 &  6892 \\
\bottomrule
\end{tabular}
\caption{The best objective value found by Ipopt with under $10^{-6}$ constraint violation for the embedded formulations.}
\label{tab:embedded-engine-obj}
\end{table}

We observe that except for the very smallest problems, namely, neural networks with 1 hidden layer and at most 10 time steps or with 3 hidden layers and 3 time steps, CPLEX fails to terminate within the allotted time limit of 3 hours. Even worse, it fails to even find a feasible solution for most problems with architectures with 3 or 5 hidden layers. This is to be expected because, except for the smallest cases, these problems can involve thousands of binary variables. With the warmstart, CPLEX is actually able to find solutions with significantly better objective values for each of the configurations. It still fails to prove optimality for any of these solutions, however, and therefore times out for the same set of problems as without the warmstart. 

Ipopt, on the other hand, always finds locally optimal solutions within the time limit, often in  seconds for problems with a small number of time steps. These solutions may be suboptimal, however, as can be seen for the single hidden layer case with 6 time steps, where the computed solution is off from the globally optimal solution by a fair amount. 

We observe that Ipopt with the warmstart solution tends to outperform Ipopt in terms of speed generally by a factor of 2. Furthermore, the objective solution tends to have a significantly smaller objective although there are a few exceptions. Surprisingly, CPLEX without warmstart finds a better solution than Ipopt does in only three problem instances. and in all three
cases Ipopt is within 0.1\% of CPLEX's globally optimal solution. With the warmstart, in terms of objective value, there is no clear winner as Ipopt produces better solutions for the 1-layer and 5-layer networks while CPLEX produces marginally better solutions for the 3-layer networks. Again however, Ipopt with warmstart takes significantly less time finding its solution within seconds for the smallest problems and minutes for all but the largest problem whereas CPLEX generally took nearly 3 hours to find its best solution.

\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{images/relu_dual_inf.png}
    \includegraphics[width=0.45\linewidth]{images/swish_dual_inf.png}
    \caption{Objective value, primal infeasibility and dual infeasibility of a sample ReLU network (left) and a sample swish network (right) over an Ipopt solve.}
    \label{fig:dual-infeas}
\end{figure}

The embedded formulation using ReLU networks illustrates the difficulty with optimizing over ReLU networks given that the functions themselves are highly nondifferentiable owing to the cusp of the ReLU activation function. We can observe from Figure \ref{fig:dual-infeas} that for the ReLU networks, there are real difficulties with finding convergence as the dual infeasibility never decreases below a certain magnitude. We see that the objective decreases and the iteration becomes feasible as primal infeasibility becomes small. Almost all instances do not converge even though they find good solutions in many instances. This type of behavior makes this formulation difficult for general use as there are not clear conditions in general for checking if the current solution at hand is ``good.'' On the other hand, the Swish networks are smooth and the algorithms converge relatively quickly as dual infeasibility decreases alongside primal infeasibility.

The amount of time taken for Ipopt to find its best solution within three hours for each embedded network formulation on each engine combustion instance is displayed in Table \ref{tab:embedded-engine-time} and the corresponding best objective values are recorded. We observe that in almost all cases, both embedded network formulations are able to find their best solution more quickly than either the MIP or MPCC formulations. However, without the warmstart, we observe that the embedded ReLU network formulation performs worse in all but a few cases with an objective value which is up to 10\% larger than the MPCC formulation objective values. With the warmstart, we find that the objective values are comparable except for the largest network which record larger objective values than the MPCC formulation. We suspect this is owing to the nondifferentiability of network confounding the solve and preventing the solver from finding finding better solutions than the warmstart solution.

The Swish network formulations cannot be directly compared to the other formulations since the neural network approximation will differ slightly. We can comment on the behavior of convergence and note that in all cases as opposed to the ReLU network formulation, the solver converges quickly to a quality solution. Perhaps due to the smoothness of the neural network, the solver can always find a good solution. In addition, we also note that unlike the MIP and MPCC formulations which grow in problem size and solving time as the neural networks grow in size, the embedded formulations do not demonstrate significant differences in solve time between the different networks since there are not additional variables and constraints for each new neural network node.

Overall, these experiments confirm our prior suspicions that solving using the MILP formulation without warmstart quickly becomes computationally intractable as the size of the neural network increases past modest architectures. Switching to the MPCC formulation of the problem offers significant speedup at the cost of losing global optimality, although when the MPCC formulation performs worse, it tends to be by only a marginal amount, and when it does better, it can be by a significant amount. The embedded formulations on the other hand provide speed and scalability, but the ReLU formulation often expresses difficulty with convergence. We also observe that significant gains can be realized in terms of both solving time and solution quality by providing a solver with a high-quality warmstart solution for all formulations.

% The time taken for each solve is presented in Table \ref{tab:fullEngineSolveTimes} and the final MIP gaps after 8 hours (28800 seconds) are shown in Table \ref{tab:fullEngineSolveGaps}. From the tables, we clearly see that these problems quickly become computationally intractable for any neural network with more than 3 layers and for problems with more than 6 time steps. 


% These results suggest that approaching the problem using the formulation as presented in (\ref{eq:optEngine}) only is feasible for small networks with small numbers of time steps. If we wished to use a 6 layer network as is done in the original work related to these drive cycles, we would be limited to solves with at most 6 time steps. Since we have drive cycles of 1500 seconds, this would limit us to only specifying the parameters for 250 second intervals.

% \begin{table}[htbp]
%     \label{tab:fullEngineSolveTimes}
%     {\caption{Time taken to solve the full problem \ref{eq:optEngine}. Each run was timed out at 8 hours (28800 seconds). Any run which achieves a time of 28800 seconds was timed out before completion.}}
%     {
%     \begin{tabular}{@{}lllllll@{}}
%     \toprule
%     \# Layers & 2 & 3 & 6 & 10 & 25 & 50 \\\midrule
%      1 &   0& 0.1& 0.1& 0.1& 0.4& 1.8 \\
%      2 & 9.3& 32.1& 4036& 28800& 28800& 28800 \\
%      3 & 103& 3282 & 26460& 28800& 28800& 28800 \\
%      4 &  132& 4232& 28800& 28800& 28800& 28800 \\
%      5 &  878 & 13020 & 28800 & 28800 & 28800 & 28800 \\
%      6 &  21126& 16512& 28800& 28800& 28800& 28800 \\ \bottomrule
%     \end{tabular}
%     }
% \end{table}


% \begin{table}[htbp]
%     \label{tab:fullEngineSolveGaps}
%     {\caption{Final MIP Gap after 8 hours of solve time. If the MIP gap is $\infty$, this means that no feasible solution was found.}}
%     {
%     \begin{tabular}{@{}lllllll@{}}
%     \toprule
%     \# Layers & 2 & 3 & 6 & 10 & 25 & 50 \\\midrule
%   1 & 0.  &    0.  &    0.  &    0.  &    0.  &    0. \\
%     2 & 0&   0&    0&    7.73&   42.68&  143.7 \\
%     3 &  0&    0&   52.38&   56.2 &  405.75&     $\infty$ \\
%     4 &  0&    0&   16.29&   45.  &   85.25&     $\infty$ \\
%      5 &   0 &    0 &  123.72& 1178.61&     $\infty$&     $\infty$ \\
%     6 &  0&   0  &  180.38&     $\infty$&     $\infty$&     $\infty$ \\ \bottomrule
%     \end{tabular}
%     }
    
% \end{table}



% \subsection{Solving the Decomposed Problem}

% Instead of solving the full problem, we use the approach described in Figure \ref{alg:decomposedAlg}. This has the benefit of using problems which are quicker to solve at the cost of having to solve more of them. Usually the time gained from solving smaller problems significantly outweighs the extra time needed to solve additional instances.

% We tabulate the average solve time for each of the subproblems in the decomposed problem in Table \ref{tab:subproblem-times}. Note that for the 6 layer network, if we still wanted to solve the problem for all 1500 time steps, we would need to take approximately $1500\cdot 14.325 \approx 21500$ seconds or approximately 6 hours. We remark that we can easily parallelize the solves to accelerate the solves. We do not take this approach and instead proceed as we do for solving the larger problem by considering larger time steps.

% \begin{table}[]
%     \centering
%     \begin{tabular}{@{}lllllll@{}}
%         \toprule
%         \# Layers & 1 & 2 & 3 & 4 & 5 & 6 \\ \midrule 
%                  & 0.0045 & 0.495 & 0.840 & 1.768 & 3.951 & 14.325 \\ \bottomrule
%     \end{tabular}
%     \caption{The average solve time for a subproblem \ref{eq:EngineSubproblem} on neural networks with varying number of layers}
%     \label{tab:subbproblem-times}
% \end{table}

% As these problems are more easily solved, we can consider smaller time steps: 3, 5, 10, 15, 30, 60, 150, 250, 500, and 750. In Figures \ref{fig:obj-2-layers}, we show the evolution of the objective and the compression ratio as the algorithm proceeds. As can be seen in Figure \ref{fig:obj-2-layers}, the size of the time step can have a large impact on the solution converged to.

% \begin{figure}
%     \centering
%     \includegraphics{images/layer_2_obj.png}
%     \caption{Objective and Compression Ratio as Algorithm in Figure \ref{alg:decomposedAlg} progresses for 2 layers.}
%     \label{fig:obj-2-layers}
% \end{figure}

% We observe that the objectives appear to converge to a certain value near time steps of about 30 seconds. This can be seen in Figure \ref{fig:obj-layer-variation}. We see that for very large time steps, we cannot hope to be close the actual emissions over the entire drive, but as we decrease our time steps to less than half a minute we approach a value which we can take to be the actual emissions.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\linewidth]{obj_variation_3.png}
%     \includegraphics[width=0.4\linewidth]{obj_variation_6.png}
%     \caption{Variation of the objective as the size of the time step changes}
%     \label{fig:obj-layer-variation}
% \end{figure}


==> OilWell.tex <==
\section{Surrogate Modeling of Oil Well Networks}

\subsection{Optimization Problem Formulation}

The next example of an optimization problem with an embedded neural network involves the operation of an offshore oil platform and is taken from \citep{grimstad2019relu}. The full optimization problem is reproduced in \eqref{eq:oil-well-problem} and the associated sets are given in Table \ref{tab:oil-well-sets}.

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{images/network.PNG}
%    \caption{Example oil well flow network. PLACEHOLDER TAKEN FROM OTHER PAPER}
%    \label{fig:oil-well-network}
%\end{figure}

\begin{table}
    \centering
    \begin{tabular}{c|l} \toprule
        Set & Description \\ \midrule 
        $N$ & Set of  nodes in the network. \\
        $N^w$ & Subset of well nodes in network. \\
        $N^m$ & Subset of manifold nodes in the network. \\
        $N^s$ & Subset of separator nodes in the network. \\
        $E$ & Set of edges in the network. \\
        $E^d$ & Subset of discrete edges that can be turned on or off. \\
        $E^r$ & Subset of riser edges. \\
        $E_i^{\text{in}}$ & Subset of edges entering node $i$. \\
        $E_i^{\text{out}}$ & Subset of edges leaving node $i$. \\
        $C$ & Oil, gas, and water. \\
        \bottomrule
    \end{tabular}
    \caption{Sets used in oil well optimization problem}
    \label{tab:oil-well-sets}
\end{table}

\begin{figure}
    \centering
    \includegraphics{}
    \caption{Example oil well network with 8 wells, 2 manifolds and 2 separators from \cite{grimstad2019relu}.}
    \label{fig:oil-well}
\end{figure}

In this problem, we have a network comprised of three sets of nodes: the wells $N^w$ which are the sources of oil, water, and gas, the manifolds $N^m$ which are connected to wells and mix incoming flows of oil, water, and gas, and the separators $N^s$ which are the sinks of all the flow. Each well is connected to each manifold by a pipeline in $E^d$ which may be turned on and off. Each manifold is then connected to a unique separator by a riser in $E^r$. A depiction of an example network with 8 wells, 2 manifolds, and 2 separators taken from \cite{grimstad2019relu} is presented in Figure~\ref{fig:oil-well}.

\begin{subequations}
    \begin{align}\label{eq:oil-well-problem}
        \dps \maxi_{y,q,p,\Delta p} & \dps \sum_{e \in E^r} q_{e,\text{oil}} &  \\
        \st & \sum_{e \in E_i^{\text{in}}} q_{e,c} = \sum_{e\in E_i^{\text{out}}} q_{e,c}, \; \forall c \in C, i \in N^m \label{eq:flow-balance}\\
          & p_j = g_e(q_{e,\text{oil}}, q_{e,\text{gas}}, q_{e,\text{wat}}, p_i), & \forall e = (i,j) \in E^r \label{eq:p-nn}\\
          & \Delta p_{e} = p_i - p_j,  & \forall e = (i,j) \in E^r \\
          & - M_e (1 - y_e) \le p_i - p_j - \Delta p_e, & \forall e = (i,j) \in E^d \label{eq:on-off1}\\
          & p_i - p_j - \Delta p_e \le M_e (1 - y_e), & \forall e = (i,j) \in E^d \label{eq:on-off2}\\
          & \sum_{e \in E_i^{out}} y_e \le 1, & \forall i \in N^w \label{eq:routing}\\
          & y_e q^L_{e,c} \le q_{e,c} \le y_e q_{e,c}^U & \forall c \in C, e \in E^d \label{eq:flow-off}\\
          & p_i^L \le p_i \le p_i^U, & \forall i \in N \label{eq:pressure-bound} \\
          & \sum_{e \in E_i^{\text{out}}} q_{e,\text{oil}} = f_i(p_i), & \forall i \in N^w \label{eq:q-nn}\\
          & \sum_{e \in E_i^{\text{out}}} q_{e,\text{gas}} = c_{e,\text{gor}} \sum_{e \in E_i^{\text{out}}} q_{e,\text{oil}}, & \forall i \in N^w \label{eq:ratio1}\\
          & \sum_{e \in E_i^{\text{out}}} q_{e,\text{wat}} = c_{e,\text{wor}} \sum_{e \in E_i^{\text{out}}} q_{e,\text{oil}}, & \forall i \in N^w \label{eq:ratio2}\\
          & p_i = p_i^s = \text{const.}, & \forall i \in N^w  \\
          & y_e \in \{0, 1\}, \forall e \in E^d
    \end{align}
\end{subequations}

We have multiple sets of variables encoding this system: $p_i$ , the pressure at each node $i$, $\Delta p_e$, the pressure drop over edge $e$, $q_{e,c}$, the flow rate of oil, gas, and water on each edge $e$, as well as binary variables $y_e$ indicating which pipelines are open. There are also a variety of constants indicating ratios, and bounds on variable which are fixed. 

Our goal in this problem is then to optimize the flow rate of oil to each of the sinks. There area variety of physical and logical constraints to encode the operation of this flow network.  \eqref{eq:flow-balance} ensures that the flow into each node matches the flow out of each node. \eqref{eq:on-off1} and \eqref{eq:on-off2} ensure that if a pipeline is open, then the difference in pressure between the two nodes is actually represented by $\Delta p_e$.  \eqref{eq:routing} ensures that each well only routes its flow to a single manifold. \eqref{eq:flow-off} bounds the flow rate of each material when pipelines are active and forces the rate to zero when inactive whereas \eqref{eq:pressure-bound} bounds the pressure at each node. \eqref{eq:ratio1} and \eqref{eq:ratio2} establish the expected ratio of flow rates of each material.

The neural networks $g_e$ and $f_i$ appear in the problem in \eqref{eq:p-nn} and \eqref{eq:q-nn} and represent nonlinear functions which predict the separator pressure and outgoing oil flow rate based on incoming flow rate and pressure respectively. There is one neural network $g_e$ for each riser edge, and one neural network $f_i$ for each well. Each is trained separately and for our particular configuration of the network, we have $2 + 8 = 10$ separate neural networks which are encoded into our problem.

The authors in \cite{grimstad2019relu} considered two different configurations of neural networks for this problem: a ``shallow'' network with few layers of many nodes and a ``deep'' network with many layers of fewer nodes. The shallow configuration had two hidden layers of 20 nodes for the well networks $f_i$ and two hidden layers of 50 nodes for the riser networks $g_e$. The deep configurations have four hidden layers of 10 nodes for the well networks and 5 layers of 20 nodes for the riser networks. All in all, this corresponds to 520 ReLU nodes. This means that the MILP formulation will have 520 binary variables in addition to the 16 binary variables $y_e$.

\subsection{Experiments}

We assessed the performance of each of our separate formulations on this particular optimization problem. We again used CPLEX for the MIP formulation and solved the problem with a time limit of 1 hour recording the best time for each neural network configuration. As this problem involves binary variables even in complementary constraint formulation, we needed to use the MINLP solver bonmin \cite{bonami2007bonmin}. We used the default branch and bound scheme with Ipopt as the NLP solver.
As no MINLP solver is currently supported on JuMP for handling both integer variables and user-defined nonlinear functions, we could not solve the problem as stated using the embedded neural network formulations. 

In order to obtain a problem which did not have binary variables, we considered fixing each of the $y_e$ to randomly either 0 or 1 for each $e \in E^d$. If we represent the neural networks using complementary constraints or using the embedded formulation, then these will be simple NLPs which we can directly solve using Ipopt as before. In our setup, we considered 10 different configurations of the binary variables, and solved them using CPLEX for the MIP formulation and Ipopt for the rest. We ran each instance until convergence or 1 hour had passed and recorded the best solution found.

\subsection{Results}

The results for the solves on the full problem are presented in Table \ref{tab:full-oil-well-problem}. We observe that in this small set of problems, the MPCC formulation outperforms the MIP formulation in both network configurations both in terms of time taken as well as objective value produced. CPLEX fails to even produce a solution for the deep neural network configuration. These are hard problems to be sure as in 3 of the 4 solves performed, the solutions found are not proven optimal.

\begin{table}
    \centering
    \begin{tabular}{c|cc|cc}
    \toprule
     &\multicolumn{2}{c}{Shallow} & \multicolumn{2}{c}{Deep} \\
    Solver    & Time (s) & Objective & Time (s) & Objective \\ \midrule
    CPLEX &  $3388^*$ & 1.271 & $3600^*$ & NaN \\
    bonmin &  $1865^*$ & 1.283 & 1275.3 & 1.304 \\
        \bottomrule
    \end{tabular}
    \caption{The time to find the best solution for each instance of the full oil well problem with a time limit of 1 hour. A * indicates that the solver could not prove the solution optimal.}
    \label{tab:full-oil-well-problem}
\end{table}

The results for the experiments performed with the binary variables fixed to arbitrary configurations are presented in Table \ref{tab:partial-oil-problem-time} which details the solve times and Table \ref{tab:partial-oil-problem-obj} which details the objective values produced.

\begin{table}
\centering
\begin{tabular}{l|rrrr|rrrr}
\toprule
    & \multicolumn{4}{c}{Shallow} & \multicolumn{4}{c}{Deep} \\
Instance &  MIP &  MPCC &  ReLU NN &  Swish NN & MIP &  MPCC &  ReLU NN &  Swish NN \\ \midrule
1 &                17.5 &                 1.8 &               10.3 &                 4.3 &             $3600^*$ &              1.6 &            16.7 &              5.9 \\
2 &                22.0 &                 1.2 &                8.2 &                10.1 &             $3600^*$ &              1.4 &            19.4 &              3.8 \\
3 &                23.9 &                 1.5 &                7.5 &                12.6 &             $3600^*$ &              1.7 &            14.2 &              7.0 \\
4 &                40.3 &                 1.5 &                6.2 &                 7.5 &             $3600^*$ &              1.4 &             7.2 &              6.0 \\
5 &                19.0 &                 1.4 &                4.0 &                 6.4 &             $3600^*$ &              1.6 &            13.0 &             11.0 \\
6 &                21.0 &                 2.1 &                3.0 &                 7.4 &             $3600^*$ &              1.7 &             7.1 &              2.8 \\
7 &               169.4 &                 1.7 &                5.4 &                 3.7 &             $3600^*$ &              1.2 &            14.1 &             21.4 \\
8 &                14.9 &                 1.5 &                5.7 &                 5.9 &             $3600^*$ &              1.4 &             7.3 &              6.8 \\
9 &                86.3 &                 1.9 &                4.3 &                 1.9 &             $3600^*$ &              1.6 &            12.1 &              5.6 \\
10 &                15.5 &                 1.7 &                5.8 &                 5.8 &             $3600^*$ &              1.5 &             5.8 &             14.0 \\
\bottomrule
\end{tabular}
\caption{Time until a solver finds the best feasible solution for each formulation and for both shallow and deep neural networks on each particular fixing of the oil well problem. A * indicates that the solver could not prove the found solution optimal.}
\label{tab:partial-oil-problem-time}
\end{table}

We observe that overall, the MPCC formulation clearly outperforms all the other formulations in terms of speed in that it is able to find solutions in about 2 seconds where the embedded network formulations take 10 to 20 seconds and the MIP formulation can take much longer. In fact, the MIP formulation fails to find a single solution for any of the instances using the deep neural network configuration which may suggest that optimization problems with deeper networks are more difficult than networks with shallow networks even if the number of nodes is the same. 

\begin{table}
\centering
\begin{tabular}{l|rrrr|rrrr}
\toprule
    & \multicolumn{4}{c}{Shallow} & \multicolumn{4}{c}{Deep} \\
Instance &  MIP &  MPCC &  ReLU NN &  Swish NN & MIP &  MPCC &  ReLU NN &  Swish NN \\ \midrule
1 &              1.231 &              1.231 &             1.231 &              1.110 &            NaN &           1.248 &          1.183 &           1.002 \\
2 &              1.228 &              1.228 &             1.228 &              1.078 &            NaN &           1.228 &          1.155 &           0.976 \\
3 &              1.219 &              1.219 &             1.219 &              1.195 &            NaN &           1.229 &          1.274 &           1.064 \\
4 &              1.264 &              1.264 &             1.264 &              1.178 &            NaN &           1.274 &          1.255 &           1.043 \\
5 &              1.182 &              1.182 &             1.182 &              1.184 &            NaN &           1.192 &          1.253 &           1.055 \\
6 &              1.252 &              1.252 &             1.252 &              1.189 &            NaN &           1.256 &          1.266 &           1.059 \\
7 &              1.229 &              1.229 &             1.229 &              1.137 &            NaN &           1.244 &          1.215 &           1.010 \\
8 &              1.207 &              1.207 &             1.207 &              1.160 &            NaN &           1.201 &          1.225 &           1.021 \\
9 &              1.239 &              1.239 &             1.239 &              1.201 &            NaN &           1.249 &          1.282 &           1.071 \\
10 &              1.263 &              1.263 &             1.263 &              1.162 &            NaN &           1.276 &          1.243 &           1.038 \\
\bottomrule
\end{tabular}
\caption{The objective value of the best feasible solution for each formulation for both shallow and deep neural networks on each particular fixing of the oil well problem. A NaN indicates that no feasible solution was found.}
\label{tab:partial-oil-problem-obj}
\end{table}

In terms of objective value, for the shallow network all formulations were able to find the global optimum in every instance relatively quickly. For the deep networks, the different formulations outperformed each other on different instances leaving no clear winner. The Swish neural network formulation also performs well although it cannot be directly compared to the other formulations since it only approximates their behavior.

Unlike the other two problems, we observed for these instances, the embedded ReLU network formulation did not have trouble with convergence and in spite of nondifferentiability, the dual infeasibility was brought down to zero signifying convergence in all instances. We postulate that the reason for the success here as compared to the other instances may be due to the simplicity of the networks: 8 of the networks are single input and single output, and so the difficulties that might emerge in multiple dimensions do not appear. As such, we do not observe a clear advantage to using the Swish networks in this scenario. Both embedded network formulations converge in much the same manner and in approximately the same amount of time.

==> single_layer.tex <==
Next, we show that the stationarity conditions of the MPCC formulation, \eqref{eq:OptiDNN-NLP}, and of the embedded formulation, \eqref{eq:OptiML}, are equivalent. To simplify the proof, we consider \eqref{eq:OptiML} with a single-layer ReLU network.  In particular, we consider the following pair of problems:
\begin{equation}\label{eq:OptiSingleReLU}
    \begin{array}{ll}
     \dps \mini_x \; & f\left(x,\max(0,W^T x+b)\right) \\
     \st        \; & c\left(x,\max(0,W^T x+b)\right) \leq 0,
    \end{array}
\end{equation}
and
\begin{equation}\label{eq:OptiSingleMPCC}
    \begin{array}{ll}
     \dps \mini_x \; & f\left(x,y)\right) \\
     \st       \; & c\left(x,y)\right) \leq 0 \\
                & 0 \leq y \; \perp \; y \geq W^T x + b.
    \end{array}
\end{equation}
In particular, we will show that generalized stationary points of \eqref{eq:OptiSingleReLU} correspond to strongly stationary points of \eqref{eq:OptiSingleMPCC}.
We start by stating the following result about generalized gradients of composite functions.

\begin{lemma}\label{lemma:GenGrad}
Consider the function $h\left(x,\max(0,W^T x+b)\right)$, where $h(x,y)$ is smooth in both arguments. Its generalized gradient is
\begin{equation}\label{eq:GenGrad}
    \partial_x h = \left\{ v | v = \nabla_x h + \hat{W} \nabla_y h, \; \hat{W} \in \partial_x \max(0,W^T x + b)\right\},
\end{equation}
where all gradients of $h$ are evaluated at the point $\left(x,\max(0,W x+b)\right)$, and where 
$\hat{W} \in \partial_x \max(0,W^T x + b)$ is a particular column scaling of $W$.
\end{lemma}

\begin{proof}
We denote the columns of $W$ by $W := [w_1 : \cdots : w_N ]$, and we distinguish three cases for each $j=1,\ldots,N$ that define a multiplier $\kappa_j$:
\begin{enumerate}
    \item $w_j^T x + b_j < 0$: Then it follows that $\max(0,w_j^T x + b_j) = \{ 0 \}$, and $\partial_x \max(0,w_j^T x + b_j)=0$, and we set $\kappa_j=0$.
    \item $w_j^T x + b_j > 0$: Then it follows that $\max(0,w_j^T x + b_j) = w_j^T x + b_j$, and $\partial_x \max(0,w_j^T x + b_j)= \{ w_j \}$, and we set $\kappa_j=1$.
    \item $w_j^T x + b_j = 0$: Then it follows that $\partial_x \max(0,w_j^T x + b_j)=\text{conv}(0,w_j)$ is the convex hull of the vectors $0$ and $w_j$, and we let $\kappa_j \in[0,1]$.
\end{enumerate}
Overall, it follows that there exists $\kappa \in [0,1]^N$, satisfying the three conditions above such that 
\begin{equation}\label{eq:DefWhat}
    \partial _x \max(0,W^T x + b) \ni  \hat{W} =  W \text{diag}(\kappa).
\end{equation}
The remainder of the proof follows by applying the chain rule to $h\left(x,\max(0,W^T x+b)\right)$.
\qed
\end{proof}

Following \cite[Theorem 6.1.1]{cla:83}, the first-order conditions of the nonsmooth problem \eqref{eq:OptiSingleReLU} can be stated in terms of condition on the generalized gradients of the Lagrangian function of \eqref{eq:OptiSingleReLU}:
\begin{equation}
    {\cal L}(x,\lambda) = f\left(x,\max(0,W^T x+b)\right) + \lambda^T c\left(x,\max(0,W^T x+b)\right).
\end{equation}
If $x^*$ is a regular local minimum of \eqref{eq:OptiSingleReLU}, then it follows that there exist multipliers, $\lambda^* \geq 0$ such that $\lambda^{*^T} c\left(x^*,\max(0,W^Tx^*+b)\right)=0$ and that
$0 \in \partial_x {\cal L}(x^*,\lambda^*)$, i.e. there exists $\lambda^* \geq 0$ and $\kappa^*$ as in Lemma~\ref{lemma:GenGrad} such that
\begin{subequations}\label{eq:GenStat}
 \begin{align}
     & 0 \geq c\left(x^*,\max(0,W^T x^*+b)\right) \; \perp \; \lambda^* \geq 0 \\
     & 0 = \nabla_x f^* + \nabla_x c^* \lambda^* + W \text{diag}(\kappa^*) \left( \nabla_y f^* + \nabla_y c^* \lambda^* \right),
 \end{align}
\end{subequations}
where $f$ and $c$ are evaluated at $x^*$.

Next, we state the definition of strong stationarity for the MPCCs  \eqref{eq:OptiSingleMPCC}, see, e.g. \cite{SchSch:00} for its general form, and then show that the two conditions are equivalent in our case.

\begin{definition}[Scheel and Scholtes,  \cite{SchSch:00}]\label{def:strongStat}
We say $(x^*,y^*)$ is a strongly stationary point of \eqref{eq:OptiSingleMPCC}, if there exist multipliers $\mu^* \geq 0$, and $\nu_1^*, \nu_2^*$ such that the following conditions are satisfied:
\begin{subequations}\label{eq:StrongStat}
 \begin{align}
     & c^* \leq 0 \; \text{and} \; 0 \leq y^* \; \perp \; y^* \geq W^T x^* + b \\
     & \mu^{*^T} c^* = 0 \\
     & 0 = \nabla_x f^* + \nabla_x c^* \mu^* + W \nu_2^* \label{eq:KKTx} \\
     & 0 = \nabla_y f^* + \nabla_y c^* \mu^* - \nu_1^* - \nu_2^* \label{eq:KKTy} \\
     & y_j^* > 0 \Rightarrow \nu_{1j}^* = 0 \; \text{and} \; y_j^* > w_j^T x^* + b_j \Rightarrow \nu_{2j}^* = 0\\
     & 0 = y_j^* = w_j^T x^* + b_j \Rightarrow \nu_{1j}^* \geq 0, \nu_{2j}^* \geq 0, \label{eq:biactive}
 \end{align}   
\end{subequations}
where all functions and gradients are evaluated at $(x^*,y^*)$, i.e. $f^* := (x^*,y^*)$ etc.
\end{definition}

We note, that the last two conditions represent the fact that the multipliers of the complementarity $\nu_{1j}^*, \nu_{2j}^*$ need only be nonnegative for biactive or degenerate complementarity constraints. We can now show that the two sets of first-order conditions, \eqref{eq:GenStat} and \eqref{eq:StrongStat}, are equivalent. 

\begin{theorem}\label{theo:EquivStat}
$x^*$ is a stationary point of \eqref{eq:OptiSingleReLU}, if and only if, $(x^*,y^*)$ is a strongly stationary point of \eqref{eq:OptiSingleMPCC} with $y^*=\max(0,W^T x^* + b)$.
\end{theorem}

\begin{proof}
Assume that $(x^*,y^*)$ is a strongly stationary point that satisfies \eqref{eq:StrongStat}. Then it follows that $y^*= \max(0,W^T x^* + b)$, and hence that $c\left(x^*,\max(0,W^T x^* + b)\right)=c(x^*,y^*) \leq 0$, which implies that $x^*$ is a feasible point in \eqref{eq:OptiSingleReLU}. Moreover, complementarity holds, i.e., $\mu^{*^T} c^* = 0$, and hence, it remains to show that $0 \in \partial_x {\cal L}(x^*,\mu^*)$. Solving \eqref{eq:KKTy} for $\nu_2^*$, and substituting into \eqref{eq:KKTx}, we obtain
\[ 0 = \nabla_x f^* + \nabla_x c^* \mu^* + W \left( \nabla_y f^* - \nabla_y c^* \mu^* - \nu_1^* \right) , \]
and it remains to be shown that there exists $\kappa \in [0,1]^N$ as in Lemma~\ref{lemma:GenGrad} such that $W \left( \nabla_y f^* - \nabla_y c^* \mu^* - \nu_1^* \right) = W \text{diag}(\kappa)\left( \nabla_y f^* - \nabla_y c^* \mu^* \right)$. We now examine each component, $j=1,\ldots,N$, of the complementarity constraint in turn:
\begin{enumerate}
    \item $w_j^T x^* + b_j < 0$: Then it follows that $y_j^*=0$, $\nu_{2j}^* = 0$, and $\nu_{1j}^*$ is not sign-constrained. It follows from \eqref{eq:KKTy} that $\nu_{1j}^*=[\nabla_y f^* - \nabla_y c^* \mu^*]_j$, and hence that $\kappa_j=0$.
    \item $w_j^T x^* + b_j > 0$: Then it follows that $y_j^*=w_j^T x^* + b_j > 0$, and hence that $\nu_{1j}^*=0$. Thus, we can set $\kappa_j=1$.
    \item $w_j^T x^* + b_j = 0 = y_j^*$: Then it follows that $\nu_{1j}^*, \nu_{2j}^* \geq 0$ from \eqref{eq:biactive}. From \eqref{eq:KKTy}, we obtain that $[\nabla_y f^* + \nabla_y c^* \mu^*]_j \geq 0$, and
    $\nu_{1j}^* \in \left[0,[\nabla_y f^* + \nabla_y c^* \mu^*]_j\right]$ corresponds to choosing $\kappa_j \in [0,1]$.
\end{enumerate}
Putting the three cases together, we see that there exists $\kappa \in [0,1]^N$ satisfying the conditions from Lemma~\ref{lemma:GenGrad} such that \eqref{eq:GenStat} holds.

% We note, that $\nabla_{2j}^* = 0$, if $w_j^T x^* + b_j < y_j^* = 0$, which means that we can replace $W$ by $\hat{W}$ in the preceding equation. Moreover, it follows that $\hat{W} \nu_1^* = 0$, whenever $\nu_1{j}^*=0$ if $y_j^*>0$ or $\hat{w}_j=0$ if $w_j^T x^* + b_j < 0$. Thus we only need to consider the degenerate case, when $y_j^* = w_j^T x^* + b_j = 0$.
% For such a degenerate index, $j$, if $(\nabla_y f^* - \nabla_y c^* \mu^*)_j \geq 0$, then it follows from \eqref{eq:KKTy} that in fact $(\nabla_y f^* - \nabla_y c^* \mu^*)_j = 0 = \nu_{1j}^* = \nu_{2j}^*$. On the other hand, if $(\nabla_y f^* - \nabla_y c^* \mu^*)_j \geq 0$, then it follows that we can chose $\nu_{1j} > 0$, and obtain the desired inclusion.

The reverse direction follows by a similar construction. \qed
\end{proof}

==> swish_tables.tex <==
\begin{table}
\centering
\begin{tabular}{lllllllll}
\toprule
Architecture &  \pbox{2cm}{Mean \\ MIP \\ Time (s)} &  \pbox{2cm}{Mean \\ MIP \\ Obj.} &  \pbox{2cm}{\# Times \\MIP \\Finds \\Opt. Sol.} &  \pbox{2cm}{\# Times \\ MIP \\ Finds \\ Feas. Sol.} &  \pbox{2cm}{Mean \\MPCC \\Time \\(s)} &  \pbox{2cm}{Mean \\MPCC \\Obj.} &  \pbox{2cm}{\# Times \\MIP \\Wins} &  \pbox{2cm}{Mean \% \\Rel. \\Diff.\\ in Obj.} \\
\midrule
784,20,10       & 1.82                & 1.79            & 100                               & 100                                & 0.34                & 1.80            & 100                 & 0.61                       \\
784,40,10       & 76.85               & 1.75            & 100                               & 100                                & 1.48                & 1.77            & 100                 & 0.95                       \\
784,60,10       & 2301.8             & 1.85            & 52                                & 100                                & 4.84                & 1.87            & 100                 & 1.04                       \\
784,80,10       & 2570.7             & 2.04            & 38                                & 100                                & 14.23               & 2.07            & 99                  & 1.24                       \\
784,100,10      & 3078.4             & 2.16            & 16                                & 100                                & 22.88               & 2.18            & 95                  & 0.94                       \\
784,20,20,10   & 106.1              & 1.20            & 100                               & 100                                & 0.82                & 1.22            & 100                 & 0.95                       \\
784,40,40,10   & 3100.0             & 1.90            & 16                                & 100                                & 4.39                & 1.77            & 98                  & 1.89                       \\
784,60,60,10   & 3513.1             & 6.85            & 5                                 & 100                                & 14.26               & 1.88            & 12                  & -41.13                     \\
784,80,80,10   & 3586.7             & 27.59           & 1                                 & 76                                 & 36.10               & 1.46            & 1                   & -77.85                     \\
784,100,100,10 & 3600             & 54.83           & 0                                 & 42                                 & 56.97               & 1.78            & 0                   & -92.98                    \\
\bottomrule
\end{tabular}
\caption{Comprehensive results for solves of the MIP formulation using CPLEX and the MPCC formulation using Ipopt}
\label{tab:adversarial-results}
\end{table}

\begin{table}
\centering
\begin{tabular}{l|rrrr|rrrr}
\toprule
    & \multicolumn{4}{c}{Shallow} & \multicolumn{4}{c}{Deep} \\
Instance &  MIP &  MPCC &  ReLU NN &  Swish NN & MIP &  MPCC &  ReLU NN &  Swish NN \\ \midrule
1 &                17.5 &                 1.8 &               10.3 &                 4.3 &             $3600^*$ &              1.6 &            16.7 &              5.9 \\
2 &                22.0 &                 1.2 &                8.2 &                10.1 &             $3600^*$ &              1.4 &            19.4 &              3.8 \\
3 &                23.9 &                 1.5 &                7.5 &                12.6 &             $3600^*$ &              1.7 &            14.2 &              7.0 \\
4 &                40.3 &                 1.5 &                6.2 &                 7.5 &             $3600^*$ &              1.4 &             7.2 &              6.0 \\
5 &                19.0 &                 1.4 &                4.0 &                 6.4 &             $3600^*$ &              1.6 &            13.0 &             11.0 \\
6 &                21.0 &                 2.1 &                3.0 &                 7.4 &             $3600^*$ &              1.7 &             7.1 &              2.8 \\
7 &               169.4 &                 1.7 &                5.4 &                 3.7 &             $3600^*$ &              1.2 &            14.1 &             21.4 \\
8 &                14.9 &                 1.5 &                5.7 &                 5.9 &             $3600^*$ &              1.4 &             7.3 &              6.8 \\
9 &                86.3 &                 1.9 &                4.3 &                 1.9 &             $3600^*$ &              1.6 &            12.1 &              5.6 \\
10 &                15.5 &                 1.7 &                5.8 &                 5.8 &             $3600^*$ &              1.5 &             5.8 &             14.0 \\
\bottomrule
\end{tabular}
\caption{Time until a solver finds the best feasible solution for each formulation and for both shallow and deep neural networks on each particular fixing of the oil well problem. A * indicates that the solver could not prove the found solution optimal.}
\label{tab:partial-oil-problem-time}
\end{table}

\begin{table}
\centering
\begin{tabular}{l|rrrr|rrrr}
\toprule
    & \multicolumn{4}{c}{Shallow} & \multicolumn{4}{c}{Deep} \\
Instance &  MIP &  MPCC &  ReLU NN &  Swish NN & MIP &  MPCC &  ReLU NN &  Swish NN \\ \midrule
1 &              1.231 &              1.231 &             1.231 &              1.110 &            NaN &           1.248 &          1.183 &           1.002 \\
2 &              1.228 &              1.228 &             1.228 &              1.078 &            NaN &           1.228 &          1.155 &           0.976 \\
3 &              1.219 &              1.219 &             1.219 &              1.195 &            NaN &           1.229 &          1.274 &           1.064 \\
4 &              1.264 &              1.264 &             1.264 &              1.178 &            NaN &           1.274 &          1.255 &           1.043 \\
5 &              1.182 &              1.182 &             1.182 &              1.184 &            NaN &           1.192 &          1.253 &           1.055 \\
6 &              1.252 &              1.252 &             1.252 &              1.189 &            NaN &           1.256 &          1.266 &           1.059 \\
7 &              1.229 &              1.229 &             1.229 &              1.137 &            NaN &           1.244 &          1.215 &           1.010 \\
8 &              1.207 &              1.207 &             1.207 &              1.160 &            NaN &           1.201 &          1.225 &           1.021 \\
9 &              1.239 &              1.239 &             1.239 &              1.201 &            NaN &           1.249 &          1.282 &           1.071 \\
10 &              1.263 &              1.263 &             1.263 &              1.162 &            NaN &           1.276 &          1.243 &           1.038 \\
\bottomrule
\end{tabular}
\caption{The objective value of the best feasible solution for each formulation for both shallow and deep neural networks on each particular fixing of the oil well problem. A NaN indicates that no feasible solution was found.}
\label{tab:partial-oil-problem-obj}
\end{table}
